Examining Gender Bias in Languages with Grammatical Gender

Recent studies have shown that word embeddings exhibit gender bias inherited from the training corpora. However, most studies to date have focused on quantifying and mitigating such bias only in English. These analyses cannot be directly extended to languages that exhibit morphological agreement on gender, such as Spanish and French. In this paper, we propose new metrics for evaluating gender bias in word embeddings of these languages and further demonstrate evidence of gender bias in bilingual embeddings which align these languages with English. Finally, we extend an existing approach to mitigate gender bias in word embeddings under both monolingual and bilingual settings. Experiments on modified Word Embedding Association Test, word similarity, word translation, and word pair translation tasks show that the proposed approaches effectively reduce the gender bias while preserving the utility of the embeddings.

==> EMNLP2019-Bias in Bilingual word embeddings/sections/abstract.tex <==
Recent studies have shown that word embeddings exhibit gender bias inherited from the training corpora. However, most studies to date have focused on quantifying and mitigating such bias only in English. These analyses cannot be directly extended to languages that exhibit morphological agreement on gender, such as Spanish and French. In this paper, we propose new metrics for evaluating gender bias in word embeddings of these languages and further demonstrate evidence of gender bias in bilingual embeddings which align these languages with English. Finally, we extend an existing approach to mitigate gender bias in word embeddings under both monolingual and bilingual settings.
%also contain gender bias and the bias propagates to bilingual word embeddings. We propose new definitions and mitigation methods of gender bias for languages with grammatical gender and bilingual word embedding. %We find gender bias also exists in the embeddings of these languages and our definitions can capture the multifaceted gender information embedded in them.
%propose new definitions of gender bias and methods to mitigate it in Spanish.% as those proposed for English word embeddings fail to adapt to languages with grammatical gender. 
%We consider using bilingual word embeddings to facilitate mitigating the bias. We also analyze and reduce bias in bilingual word embeddings. 
Experiments on modified Word Embedding Association Test, word similarity, word translation, and word pair translation tasks show that the proposed approaches effectively reduce the gender bias while preserving the utility of the embeddings.
%And evaluation on word translation and sentence translation for bilingual word embeddings shows that our mitigation approaches preserve the 


==> EMNLP2019-Bias in Bilingual word embeddings/sections/analysis.tex <==
% \begin{figure}
% 	\includegraphics[width=\columnwidth]{figures/pca.png}
% 	%\vspace{-1em}
% 	\centering
% 	\caption{Percentage of variance explained in PCA of vector differences for gender-definition pairs when constructing the gender direction in Spanish.}~\label{fig:pca}
% 	%\label{fig:boat1}
% 	%\vspace{-2em}
% \end{figure}
\label{sec:mweat}
%This section investigates gender bias in Spanish word embeddings and English-Spanish bilingual word embeddings. %We first evaluate the bias in Spanish showing that in such a language with grammatical gender, word embeddings still exhibit societal stereotypes by constructing semantic and grammatical gender directions. Then we analyze the projection of different types of words on these two directions. 
%As mentioned earlier, gender information in Spanish is far different from that in English, so we cannot directly adopt the gender direction from English embeddings based on previous work. 
This section discusses how to analyze bias in embeddings of gendered languages and bilingual word embeddings.  
%we first define gender directions. Then we quantify gender bias in the embeddings by analyzing the projections of words on these directions. Finally, we analyze and quantify gender bias in bilingual word embeddings. %We analyze use Spanish word embeddings
% KW: you repeat this too many times. 

\subsection{Bias in Gendered Languages} \label{bias_ggl}
%\paragraph{Gender Directions}
%In Spanish word embeddings, we propose a new way to define gender directions to evaluate the bias. Specifically, 
In gendered languages, all nouns are assigned a gender class. However, inanimate objects (e.g., water and spoon) do not carry the meaning of male or female. 
%We want to address this type of grammatical gender information, which should not be considered as bias, and separate it from the gender inclination in semantics.
%\kw{need a short paragraph here to motivate why we need these two directions. Say, for example, in Spanish, spoon, water are marked with gender but they are not related to male/female. However, when training the embedding space, these words will get involved and ...}
To address this issue, we define two gender directions: (1) \textit{semantic gender}, which is defined by a set of gender definition words (e.g., man, male, waitress) and (2) \textit{grammatical gender}, which is defined by a set of masculine and feminine nouns (e.g., water, table, woman). Most analysis of gender bias assumes that the language (e.g,. English) only has the former direction. However, when analyzing languages like Spanish and French, considering the second is necessary. We discuss these two directions in detail as follows.

%used to measure the semantically male or female inclination of the word. The other is for \textit{grammatical gender}, which is used to capture the inherently carried gender attribute of the word. We claim that the semantic gender direction is enough for measuring bias in English embeddings since English does not have grammatical gender. But for languages like Spanish and French, the second type of gender direction is necessary.
%grammatical gender leads to another type of gender information besides semantic gender so we need two directions. 
%We constrain that the two directions are orthogonal to each other to better distinguish between the two types of gender information. For all nouns in gendered languages, we do not take the inclinations along the grammatical gender direction as bias and only focus on the bias shown in the semantic gender. 
%

\paragraph{Semantic Gender} Following~\citet{kaiwei}, we collect a set of gender-definition pairs (e.g., ``mujer'' (woman) and ``hombre'' (man) in Spanish). Then, the gender direction is derived by conducting principal component analysis (PCA)~\cite{jolliffe2011principal} over the differences between male- and female-definition word vectors. Similar to the analysis in English, we observe that there is one major principal component carrying the meaning of gender in French and Spanish and we define it as the semantic gender direction $\vec{d}_{PCA}$.

\paragraph{Grammatical Gender} 
The number of grammatical gender classes ranges from two to several tens~\cite{corbett1991gender}. To simplify the discussion, we focus on noun class systems where two major gender classes are feminine and masculine. However, the proposed approach can be generalized to languages with multiple gender classes (e.g., German). To identify grammatical gender direction, we collect around 3,000 common nouns that are grammatically masculine and 3,000 nouns that are feminine.
Since most nouns (e.g., water) do not have a paired word in the other gender class, we do not have pairs of words to represent different grammatical genders. Therefore, instead of applying PCA, we learn the grammatical gender direction $\vec{d_g}$ by Linear Discriminant Analysis (LDA)~\cite{fisher1936use}, which is a standard approach for supervised dimension reduction. The model achieves an average accuracy of 0.92 for predicting the grammatical gender in Spanish and 0.83 in French with 5-fold cross-validation. %We also verify the computed direction by using another classifier: linear SVM, and find that the direction from SVM has a cosine similarity of 0.99 with the direction from LDA. \kw{need a sentence and to elaborate what do you mean by verifying with linear SVM. Also, it's unclear what do you mean by direction from SVM and what is the setting here.}
%Additionally, we also train a linear SVM to predict the binary grammatical gender and find that 
%\kw{Can you also mention the result of LDA? You can say, linear discriminate analysis is a standard approach for supervised dimension reduction. Alternatively, we can also train a linear classifier to identify the direction to separate two or more classes of vectors. Then, mention the results of both.}
%\kh{You can mention the term $\vec{d_g}$ here.}
%We get the centroid of the male and female clusters and use the difference between these two as the \grg~direction. 

 %As an example, Figure \ref{fig:pca} shows the percentage of variance explained by each component for Spanish fastText~\cite{fasttext} word embeddings pre-trained on Wikipedia. 

Comparing $\vec{d}_{PCA}$ with $\vec{d}_g$, the cosine similarity between them is 0.389, indicating these two directions are overlapped to some extent but not identical. This is reasonable because words such as ``mujer (woman)'', ``doctor (female doctor)'' are both semantically and grammatically marked as feminine. 
To better distinguish between these two directions, we project out the grammatical gender component in the computed gender direction to make the semantic gender direction $\vec{d}_s$ orthogonal to the grammatical gender direction:
\begin{equation*}
    \vec{d_s} = \vec{d}_{PCA} - \left \langle \vec{d}_{PCA} , \vec{d}_{g} \right \rangle \vec{d}_{g},
\end{equation*}
where $\left \langle \vec{x},\vec{y}  \right \rangle$ represents the inner product of two vectors. 
%Along this direction, masculine and feminine forms of one occupation word should have similar distances to male concepts and female concepts respectively, i.e., symmetric with respect to the gender-neutral position, otherwise they show bias. 
\paragraph{Visualizing and Analyzing Bias in Spanish}
We take Spanish as an example and analyze gender bias in Spanish fastText word embeddings~\cite{fasttext} pre-trained on Spanish Wikipedia. For simplicity, we assume that the embeddings contain all gender forms of the words.
To show bias, we randomly select several pairs of gender-definition and occupation words as well as inanimate nouns in Spanish and visualize them on the two gender directions defined above.
%We enclose masculine and feminine forms of the occupation words as well as the Spanish word for ``he'' (``\'{e}l'') and ``she'' (``ella'') by dotted blue and red lines, respectively. 

Figure \ref{fig:viz_2directions} shows that the inanimate nouns lie near the origin point on the semantic gender direction, while the masculine and feminine forms of the occupation words are on the opposite sides for both directions.
However, while projections of occupation words on the grammatical gender direction are symmetric with respect to the origin point, they are asymmetric when projected on the semantic gender direction. 
%\kh{Are the neutral grammatical gender position and neutral semantic gender position the same position?}
Along the semantic gender direction, female occupation words incline more to the feminine side than the male occupation words to the masculine side. This discrepancy shows that the embeddings carry unequal information for two genders. 
%difference in the gender information carried by the two forms of the same words and conforms our definition for gender bias in Spanish. %Besides, we also find some interesting cases like ``\'{e}l'' (he) and ``cient\'{i}fica'' (feminine scientist) that are different from rest of the words in their group. We speculate that their extreme frequencies (too high or too low) lead to this phenomena.
%For inanimate nouns, their grammatical gender a

%are categorized well on the grammtical gender dir

%we find that most of them lie near the origin points on the semantic gender direction, but words with different grammatical gender are on different sides when projected on the grammatical gender direction.


%\kw{wee need to show numbers here using our quantitative metrics. }
\paragraph{Quantification of Gender Bias}
%With the grammatical gender and the semantic gender directions defined, we can formally quantify gender bias in gendered languages. 
To quantify gender bias in English embeddings, \citeauthor{caliskan2017semantics}~(\citeyear{caliskan2017semantics}) propose Word Embedding Association Test (WEAT), which measures the association between two sets of target concepts and two sets of attributes. Let $X$ and $Y$ be equal-sized sets of target concept embeddings (e.g., words related to mathematics and art) and let $A$ and $B$ be sets of attribute embeddings (e.g., male and female definition words such as ``man'', ``girl''). Let $\cos(\vec{a},\vec{b})$ denote the cosine similarity between vectors $\vec{a}$ and $\vec{b}$. The test statistic is a difference between sums over the respective target concepts,  \begin{equation*}
    s(X,Y,A,B)=\sum_{\vec{x}\in X}s(\vec{x},A,B) - \sum_{\vec{y}\in Y}s(\vec{y},A,B),
\end{equation*}
where $s(\vec{w},A,B)$ is the difference between average cosine similarities of the respective attributes,
%KW: Why cite this paper here? ~\cite{may2019measuring}, %$s(w,A,B) = \text{mean}_{a \in A} \cos (\vec{w},\vec{a})-\text{mean}_{b \in B} \cos (\vec{w},\vec{b})$~\cite{may2019measuring}.
 \begin{equation*}
         s(\vec{w},A,B) \!=\! \frac{1}{|A|}\!\sum_{\vec{a} \in A} \cos (\vec{w},\vec{a}) - \frac{1}{|B|}\!\sum_{\vec{b} \in B} \cos (\vec{w},\vec{b}).
 \end{equation*}
 %\kw{Can you add a short description about WEAT here and give example of X, A, B. Then, we can say the definition can be used to test the bias for inanimate nouns, but cannot be used for words have both gender forms such as occupation words. Then discuss how to extend this definition. }

\begin{figure}
	\includegraphics[width=\columnwidth]{figures/viz_2directions_new.pdf}
	%\vspace{-1em}
	\centering
	\caption{Projections of selected words in Spanish on grammatical and semantic directions with masculine nouns in blue and feminine nouns in red. We find that: (1) Most inanimate nouns (e.g., map, spoon; enclosed by black dotted lines) lie near the origin point of the semantic gender axis; (2) Masculine definition and occupation words (blue dotted lines) lie in the masculine side for both gender directions and so do feminine words (red dotted lines). But the feminine words are farther on the feminine side on the semantic gender direction compared to masculine words.}~\label{fig:viz_2directions}
	%\kh{(1) Can we also plot the neutral point? (2) Maybe we need to carefully choose the examples. Now all the common nouns lie on the feminine side. Does it mean there is bias for the common nouns? 
	%\label{fig:boat1}
	%\vspace{-2em}
\end{figure}

In the following, we extend the definition to quantify individual words in gendered languages. 
We consider two types of words. One is \textit{inanimate nouns}, like ``agua'' (water, feminine). They are assigned as either a masculine or feminine noun.  The other is \textit{animate nouns} that usually have two gender forms, like ``doctor'' (male doctor) and ``doctora'' (female doctor).\footnote{Note that some animate nouns in certain languages, like ``m\'{e}decin'' (male doctor) in French, only have one gender form. We omit such cases in this paper for the sake of simplicity. }  

For inanimate nouns that should not be semantically leaning towards one gender, we can quantify the gender bias for word $w$ simply using WEAT,
\begin{equation*}
    \text{b}_w = \left |s(\vec{w},A,B)\right|,
\end{equation*}
which measures the association strength of the word $w$ with the gender concepts. 
%Let $A$ contain male-definition words like ``man'' and ``boy'' and let $B$ contain female-definition words like ``woman'' and ``girl''. 
The larger $\text{b}_w$ is, the stronger its association with the gender concepts.

For nouns with two gender forms, we test if their masculine ($\vec{w}_m$) and feminine ($\vec{w}_f$) forms are symmetrical with respect to gender definition terms.
%due to grammatical gender, masculine words are naturally associated with male-definition terms more than female-definition terms and vice versa. Thus, we modify WEAT to compare the association strengths for masculine occupation words with male attribute words and for feminine occupation words with female attribute words. For example in Spanish, let $w_m$ be ``profesor'' (male professor) and $w_f$ be ``profesora'' (female professor). And $A$ and $B$ are defined similarly as before. We then define the bias as
\begin{equation}
\label{eq:mweat}
    \text{b}_w = \left |\left |s(\vec{w}_m,A,B)\right | - \left |s(\vec{w}_f,A,B)\right |\right |.
\end{equation}
The larger the value is, the larger gender bias presents. 
For example, if ``doctor'' (male doctor) leans more toward to masculine (i.e., close to masculine definition words like ``el'' (he) and far away from feminine definition words like ``ella'' (she)) than ``doctora'' leans toward to feminine, then embeddings of ``doctor'' and ``doctora'' are biased. We will discuss detailed quantitative analysis using this metric in Section~\ref{experiments}.
%is closer to ``el'' (he) than  ``doctora''
%which quantifies the absolute difference between the association strength of masculine animate nouns with male concepts and that of feminine animate nouns with female concepts. 
%The larger the value is, the larger discrepancy between of the same word. The quantification results are shown in %We then treat the absolute value of the sum of differences between mean cosine similarities of the two gender attributes for these occupation words $\left |\sum_{x\in X}s(x,A,B)\right |$ as the association of male occupation target concepts $X$ with the gender attributes. Similarly, we use $\left |\sum_{y\in Y}s(y,A,B)\right |$ as the association of female occupation words with the gender attributes. Finally our test statistic is 
%\begin{equation*}
   %\left | \left |\sum_{x\in X}s(x,A,B)\right | - \left |\sum_{y\in Y}s(y,A,B)\right | \right |,
%\end{equation*}
%which measures the difference in the association strength for two target sets with the two attribute sets occupation words. We then calculate the one-side p-value of the permutation test.

%We also show two exceptions: ``perfume'' (perfume, grammatically masculine) and ``flor'' (flower, grammatically feminine), which are leaning towards the feminine semantic gender. Their positions show that the two directions are able to distinguish between grammatical gender and semantic gender in Spanish and provide a way to measure two types of gender information. 
%\kh{Do we need to mention these two exceptions? I know these two exceptions can justify that the gender direction indeed captures something. But now in the figure, we have 6 common nous and 2 of them are exceptions. It is not so convincing for me. Maybe we can remove the exceptions and put more common words.}

\begin{figure}
	\includegraphics[width=\columnwidth]{figures/viz_bilingual_before.pdf}
	%\vspace{-1em}
	\centering
	\caption{Projections of occupation words on the semantic gender direction in two gender forms (blue for male and red for female) in Spanish, the original English word (grey), and the bias-mitigated version of the English word (black with ``*''). We find that feminine occupations are farther away from the English counterparts as well as the neutral position (indicated by the vertical line) compared to masculine words.}~\label{fig:viz_bilingual_before}
	%\label{fig:boat1}
	%\vspace{-2em}
\end{figure}
\subsection{Bias in Bilingual Word Embeddings}
%\kw{need to motivate why we want to analyze bilingual embedding. Probably, you can use the machine translation as example to motivate this. }
%After analyzing gender bias in word embeddings of gendered languages, we also define bias in bilingual word embeddings that align a grammatical gender language like Spanish with a genderless language like English. 
Bilingual word embeddings are used widely in tasks such as multilingual transfer. It is essential to quantify and mitigate gender bias in these embeddings to avoid them from affecting downstream applications. We focus on bilingual word embeddings that align a grammatical gender language like Spanish with a language without grammatical gender like English. The definitions of the two gender directions are similar: we construct the grammatical gender direction using the same sets of words in the gendered language since the other language does not mark grammatical gender. We combine the gender-definition words for both languages and remove the grammatical gender component to get the semantic gender direction similarly. 

We use bilingual word embeddings from MUSE~\cite{conneau2017word} that align English and Spanish fastText embeddings together in a single vector space. Figure~\ref{fig:viz_bilingual_before} shows the projections of 5 occupation words on the semantic gender direction. First, we notice that the embeddings of some English occupations are much closer to one gender form than the other in Spanish. For example, ``nurse'' in English is closer to ``enfermera'' (female nurse) than ``enfermero'' (male nurse) in Spanish. We further separate out the bias in English embedding in the analysis by mitigating the English embeddings using ``hard-debiasing'' approach proposed in~\citet{kaiwei} and aligning Spanish embedding with the bias-reduced English embedding (words annotated with ``*''). Results in Figure~\ref{fig:viz_bilingual_before} demonstrate another type of gender unequal in bilingual embedding: %Each occupation word has 4 versions: the masculine form in Spanish in blue, the feminine form in Spanish in red, the English word in grey, and the English word after ``hard-debiasing'' proposed by~\citet{kaiwei} in black with suffix ``\_de''. We find that the projections of ``debiased'' English words are close to the origin point but each occupation shows a different small inclination.
masculine occupation words are closer to the corresponding English occupation words than the feminine counterparts. This result aligns with the observation in Figure~\ref{fig:viz_2directions}. 

%all occupation words in the feminine form are farther away from the English occupations and the neutral position. This asymmetry is also shown in Figure~\ref{fig:viz_2directions} and matches the observation that the English occupation words like ``lawyer'' are closer to the masculine form of the same occupations (``abogado'') in Spanish as shown in Section~\ref{intro}. %The discrepancy is harmful for downstream applications that use bilingual word embeddings like machine translation as occupations in English will have a higher chance of being translated into the male form in gendered languages. 

%\kw{It is unclear to me what the following paragraph want to analysis. Also, we need to demonstrate the results somewhere to demonstrate this proposed metric. }

More quantitative analyses about gender bias in bilingual embedding will be discussed in 
%The quantification method of gender bias in bilingual word embeddings can simply be the sum of the quantification of bias for English words and gendered languages discussed in 
Section~\ref{bilingual_exp}.
%However, since words from genderless languages are aligned in the same space, we can treat their projections as the anchor points for the corresponding word pairs in gendered languages. For example, the projection of the embedding of ``engineer'' can be the anchor point for two gender forms of engineer in Spanish: ``ingeniera'' (female) and ``ingeniero'' (male). To minimize the influence of bias in English word embeddings, we use the bias-mitigated version of English embeddings.
%slightly different from the monolingual setting, mainly because we consider the projection of the corresponding mitigated English occupation word as the anchor position instead of the origin point. This is because for bilingual word embeddings, all words are in the same space and we can use previous approaches to mitigate English words and treat it as the gender-neutral position for the occupation pairs in languages with grammatical gender.
%\kh{I think it is somehow tricky. If we do not use the neutral point to quantify the bias, why do we call it "neutral" point?}

  %The observation of feminine words are farther away from the anchor point also explains for the lower similarity score and ranking for some occupation words in feminine form for the cross-lingual analogy task.\jy{Where does the 'lower similarity score and ranking' come from? } We will discuss more about this evaluation method in Section~\ref{bilingual_exp}.
%\kh{In the previous paragraph, you say we don't use original point to quantify the bias. But in this paragraph, you use original point to explain the bias. It looks like a contradiction. Also, sometimes you use term "original point" and sometimes use term "neutral position". It will better if the term can be consistent.}

%\kw{it is unclear what messages we want to send in this paragraph. We need to discuss thing one by one. I think what you can do is first show Figure~\ref{fig:viz_bilingual_before}. And, say when aligning Spanish with English, we can see some English word align to female version of the occupations, and vise verse. Then, say, we want to reduce the effect of gender bias in English. Then we aligned it with the debiased English embedding, and found another type of bias...} 

==> EMNLP2019-Bias in Bilingual word embeddings/sections/bilingual_table.tex <==

\begin{table*}[ht]
\centering
%\small
\begin{tabularx}{\linewidth}{c|c||c||c|c|c|c|c}
Task  & Metric               & Original                & Shift\_Ori              & Shift\_EN               & De-Align                & Hyrid\_Ori              & Hyrid\_EN               \\ \hline
\multicolumn{8}{c}{Word Translation} \\
\hline
EN$\rightarrow$ES & P@1/P@5     & 79.2/89.0          & \textbf{80.7/90.3}  & \textbf{80.7/90.3}  & 76.5/88.9          & \textbf{80.7/90.3}  & \textbf{80.7/90.3}  \\
ES$\rightarrow$EN & P@1/P@5     & 79.2/89.0          & 79.2/89.0           & 79.2/89.0           & \textbf{80.1/90.7} & 79.2/89.0           & 79.2/89.0           \\
%EN-ES--ST--P@1/5/10     & 49.0/59.5/63.4          & 46.1/56.8/60.3           & 46.1/ 56.8/60.4          & \textbf{50.0/61.0/64.0} & 46.1/56.8/60.3           & 46.1/56.8/60.3           \\
%ES-EN--ST--P@1/5/10     & 46.7/58.6/62.5          & 44.9/55.8/60.1           & 44.9/55.8/60.1           & \textbf{50.2/60.8/64.9} & 44.8/55.7/60.1           & 44.8/55.7/60.1           \\ \hline
EN$\rightarrow$FR &P@1/P@5     & 78.2/89.4          & \textbf{79.9/91.1} & \textbf{79.9/91.1}  & 74.3/87.8          & \textbf{79.9/91.1} & \textbf{79.9/91.1} \\
FR$\rightarrow$EN &P@1/P@5     & \textbf{76.1/88.1} & \textbf{76.1/88.1}  & \textbf{76.1/88.1} & 74.4/87.2          & \textbf{76.1/88.1}  & \textbf{76.1/88.1}  \\ \hline
%EN-FR--ST--P@1/5/10     & \textbf{43.4/53.7/57.6} & 40.8/50.8/54.9           & 40.8/50.8/54.9           & 34.1/45.6/50.5          & 40.8/50.8/54.9           & 40.8/50.8/54.9           \\
%FR-EN--ST--P@1/5/10     & \textbf{42.3/53.8/58.0} & 39.8/50.9/55.6           & 39.8/50.9/55.6           & 34.7/46.3/50.7          & 39.8/50.9/55.6           & 39.8/50.9/55.6          
\multicolumn{8}{c}{Word Pair Translation} \\ 
\hline
\multirow{4}{*}{EN$\rightarrow$ES} & ASD        & 0.1082                  & 0.0961                   & 0.0961                   & 0.0827                  & \textbf{0.0755}          & 0.0772                   \\
 & F\_MRR & 0.2073                  & 0.2507                   & 0.2507                   & 0.2919                  & 0.3450          & 0.3150                   \\
 & M\_MRR   & 0.6940                  & 0.6766                   & 0.6766                   & 0.6775                  & 0.6398          & 0.6696                   \\
 & MRR Diff   & 0.4867                  & 0.4259                   & 0.4259                   & 0.3856                  & \textbf{0.2949}          & 0.3546                   \\ \hline
\multirow{4}{*}{EN$\rightarrow$FR}  & ASD          & 0.1208                  & 0.1048                   & 0.1082                   & 0.0892                  & \textbf{0.0735}          & 0.0805                   \\
 & F\_MRR & 0.1663                  & 0.2101                   & 0.1943                   & 0.2679                  & 0.3128          & 0.2975                   \\
 & M\_MRR   & 0.6549                  & 0.6313                   & 0.6419                   & 0.6610                  & 0.6393         & 0.6467                   \\
 & MRR Diff   & 0.4886                  & 0.4212                   & 0.4476                   & 0.3931                  & \textbf{0.3265}          & 0.3492                   \\ 
\end{tabularx}
\caption{Results on word translation and word pair translation based on Spanish-English and French-English bilingual embeddings. 
%We calculate the average cosine similarity difference (ASD) for two gender forms from the cross-lingual analogy task (CLAT) and compute the mean reciprocal ranks (MRR) for female and male occupation words and their difference. 
We find that the original bilingual embeddings have a large discrepancy between the two genders, indicated by the average cosine similarity difference (ASD) and mean reciprocal ranks (MRR) difference. After applying the mitigation methods, both ASD and MRR difference drop. }%
\label{tab:bilingual_results}
\end{table*}
%\kw{please describe your key observation here. Especially explain the implication of the p-value}

==> EMNLP2019-Bias in Bilingual word embeddings/sections/conclusion.tex <==
We analyze gender bias in the embeddings of languages with grammatical gender and bilingual word embeddings that align such a language with a language without grammatical gender. 
%We find that gender bias indeed exists in both word embeddings for languages with grammatical gender and bilingual word embeddings. We introduce new definitions to quantify gender bias and propose new methods to mitigate such bias in the embeddings. 
We propose new methods to evaluate and mitigate gender bias for languages with grammatical gender and bilingual word embeddings and results show that our methods can mitigate gender bias while preserving the quality of original embeddings.
%\kw{we don't have to repeart what we did in the paper and you can shorten this part to just one or two sentences}
%We conduct analysis and mitigation of gender bias in Spanish and English-Spanish bilingual word embeddings. We introduce new definitions to measure and quantify bias in Spanish, analyze phenomena for both grammatical and semantic gender, and design methods to mitigate bias. We show that the proposed method of combining mitigating before alignment and post-processing by shifting along the semantic gender direction efficiently closes the gap between the two gender forms in Spanish as well as English-Spanish bilingual word embeddings. 

Directions for future work include testing monolingual and bilingual word embeddings on downstream tasks like machine translation to measure bias and also test the performance for mitigation methods. Moreover, the number of noun classes for other languages with grammatical gender ranges from two to several tens~\cite{corbett1991gender} and future work can extend methods proposed in this paper to address grammatical gender in languages with more gender forms.

==> EMNLP2019-Bias in Bilingual word embeddings/sections/experiments.tex <==
\input{sections/mono_table.tex}

%\kw{Please reorganize this section. A better organization is 4.1: setting, data, configuration. 4.2 monolingual experiments. Discuss the tasks and then results. 4.3. bilingual experiments. Discuss the tasks and show results. 4.4 correlation of Gender bias in different languages. }
%We conduct experiments to quantify gender bias in ES word embeddings and compare the results before and after our mitigation methods. We again use ES fastText embeddings and MUSE bilingual embeddings.
%In this section, we first discuss the choice of which words to mitigate bias. Then we describe our experiments in the monolingual and the bilingual settings. 
We evaluate gender bias mitigation methods in both monolingual and bilingual settings and 
test the utility of the bias-reduced embeddings in word-level translation tasks~\citet{conneau2017word}.
%the embeddings of gendered languages and bilingual embeddings. 
%Note that in monolingual experiments, we can use embeddings of a genderless language to help mitigate the bias. 
%For both monolingual and cross-lingual experiments, we propose new metrics to evaluate gender bias before and after mitigation, for which five methods are used. 
%We also test the utility of the embeddings following the evaluation tasks described in ~\citet{conneau2017word}. And lastly, we will present our findings on the correlation of gender bias in differen languages.
%\subsection{Evaluation Methods}
%\subsection{Mitigation Word Choice} \label{word_choice}
%\kw{I'm not sure what do you want to say in this sentence}Generally, given a set of gender-definition words like ``aunt'' and ``uncle'', we want to mitigate the gender stereotype in the embeddings of all other words and our mitigation methods can be applied to all words. 
Following other analyses on gender bias~\cite{kaiwei,caliskan2017semantics}, we quantify the gender bias based on a set of animate nouns including occupations and gender-definition words. These words are representative to the major challenge when quantifying and mitigating gender bias.
Different from previous analyses in English, most occupation words in gendered languages have more than one forms and their embeddings are inherently different from each other due to morphological agreement. % \kw{check this paragraph}

%However, note that our approach is general and can calibrate the vectors of any given set of words.
%to mitigate the gender bias. In our experiment, we consider using a set of animate nouns including occupations and gender-definition words as examples because these words are representative to the major challenge when we analyze the gender bias in gendered languages. Note that different from English, most occupation words in these languages have more than one forms and their embeddings are inherently different from each other due to morphological agreement. % \kw{check this paragraph}

%For our experiments, we provide a set of occupation words as examples and mitigate gender bias for their embeddings.\kw{can we say we calibrate their word vectors to mitigate gender bias?} We claim that occupation words in languages with grammatical gender present the main challenge for bias analysis and mitigation since they mostly have more than one gender forms and the embeddings are inherently different from English embeddings due to morphological agreement. %\kw{We should first describe how general our approach is, then say we use occupation words as example.}
\subsection{Data and Configuration}
We apply the proposed mitigation methods on Spanish-English and French-English bilingual embeddings from MUSE~\cite{conneau2017word} that align the fastText monolingual embeddings pre-trained on Wikipedia corpora together in a single vector space. We collect 58 occupation words in Spanish from the occupation list provided by~\citet{font2019equalizing} and 23 in French (some occupations in French do not distinguish between two forms) for the bias mitigation experiments. We use WEAT word lists from~\citet{caliskan2017semantics} for male and female attribute words for our WEAT experiments and translate them to Spanish and French. For the word pair translation task, we use 7 common adjectives and pair every adjective with each occupation, resulting in 406 pairs for Spanish and 161 for French. 

\subsection{Monolingual Experiments}
%\subsubsection{Bias Test}
%\kw{As I mentioned earlier, I think you want to move this definition to the section of quantifying bias as this is part of quantitative metric we proposed. } 
\paragraph{Modified Word Embedding Association Test (MWEAT)} 
As discussed in Section \ref{sec:mweat}, we evaluate the gender bias using modified WEAT and we treat the absolute value of the sum of differences between mean cosine similarities of the two gender attributes for these occupation words $\left |\sum_{\vec{x}\in X}s(\vec{x},A,B)\right |$ as the association of male occupation target concepts $X$ with the gender attributes. Similarly, we use $\left |\sum_{\vec{y}\in Y}s(\vec{y},A,B)\right |$ as the association of female occupation words with the gender attributes. Finally our test statistic is 
\begin{equation*}
   \left | \left |\sum_{\vec{x}\in X}s(\vec{x},A,B)\right | - \left |\sum_{\vec{y}\in Y}s(\vec{y},A,B)\right | \right |,
\end{equation*}
which measures the difference in the association strength for two target sets with the two attribute sets occupation words. We then calculate the one-side p-value of the permutation test.
%We compare the two association scores. If the difference is large, then one  target set associates with that gender more than the other, indicating the gap in gender information carried by two forms. 

\input{sections/bilingual_table.tex}

%\paragraph{Word Analogy Case Studies}

%\subsubsection{Utility Test}
\paragraph{Word Similarity}
We test the quality of the embeddings after mitigation on the SemEval 2017 word similarity task~\cite{camacho2017semeval} for monolingual embeddings. This task evaluates how well the cosine similarity between two words correlates with a human-labeled score for which we report the Pearson correlation score.

\begin{figure}
	\includegraphics[width=\columnwidth]{figures/viz_bilingual_after.pdf}
	%\vspace{-1em}
	\centering
	\caption{Projections of occupations words on the semantic gender direction after hybrid mitigation with origin as the anchor point. The two forms of occupations are a lot more symmetric.}~\label{fig:viz_bilingual_after}
	%\label{fig:boat1}
	%\vspace{-2em}
\end{figure}
%\kw{you can remove the following sentence to save space}This section analyzes our experimental results in both monolingual and bilingual settings for Spanish and French word embeddings. 
\paragraph{Results}
Table~\ref{tab:mono_results} shows that Hybrid\_Ori significantly decreases the difference of association between two genders as indicated by MWEAT--Diff and p-value. Other methods only show marginal mitigation effects in terms of p-value.
%We surprisingly find a large gap between using origin and mitigated English as anchor point for hybrid methods. This possibly is because that aligning the mitigated English words has redundant effects with shifting shifting with origin point embeddings  
We also find that the performance of our mitigation methods on word similarity is largely preserved as indicated by the Pearson correlation scores. 
%\paragraph{Downstream Tasks}
\subsection{Cross-lingual Experiments} \label{bilingual_exp}
\paragraph{Word Translation}
We use word translation to examine whether our mitigation approaches preserve the utility of the bilingual word embediddings. This task aims to retrieve the translation of a source word in the target language. We use the test set provided by~\citet{conneau2017word}, which contains 200,000 randomly selected candidate words for 1,500 query words. We translate a query word and report the precision at $k$ (i.e., 
fraction of correct translations that are ranked not larger than $k$) by retrieving its $k$ nearest neighbours in the target language. 
We report both results with $k = 1$ and $k=5$.
%\subsubsection{Bias Tests}
%\kw{How about we call it word pair translation by analogy? You can put it after the word translation and say beyond test single word translation, we consider this and provide some reasons (e.g., because it also provide hint based on grammar as in the example you show).}
\paragraph{Word Pair Translation by Analogy}
We propose a word pair translation task to evaluate the bias in gendered languages. In languages with grammatical gender, word forms of articles and adjectives need to agree with the gender of nouns they are associated with. For example, the word ``good'' has two forms in Spanish: ``bueno'' (masculine form) and ``buena'' (feminine form). Following the notion of analogy, we design an evaluation task to test how bilingual word embeddings translate an English occupation with the presence of another word.
Specifically, given an English word $E_i$ (a noun, an adjective or a verb), an English occupation word $E_o$, and the corresponding Spanish/French translation $S_i$ of $E_i$,
we adopt the analogy test ``$E_i$:$E_o$ = $S_i$:?'' (e.g., ``good:doctor = buena: ?'')  to rank all the words $S_o$ in Spanish/French based on the cosine similarity: $\cos(S_o, E_o - E_i + S_i)$. Ideally, the correct translation of $E_o$ that agree with gender of $S_i$ should be ranked on the top (``doctora'' in the above example). Quantitatively, we use the mean reciprocal ranks (MRR) to evaluate the performance of the ranking. If the bilingual embedding is not biased, the model should perform similarly on answering the translation of masculine and feminine occupations. Based on this, we use the gap between the performances on two form of genders to quantify the bias in the bilingual embedding space. Besides, we also report the average cosine similarity difference (ASD) of occupation words between two different gender forms.

%This task compares the similarity scores and rankings of masculine and feminine forms of the correct Spanish occupation word $S_o$. The task follows the notion of an analogy ``A:B = C:?'', where 
%in Spanish with the word in English to see whether the embedding of one form is closer to that in the mitigated English embeddings. %We build such dataset as in Spanish, adj and verb don't have any gender information. In total, there are xxx instances in this dataset.
%Based on this, we can evaluate how differently the masculine and feminine occupation words perform in this task. 
%The performance is evaluated by the average similarity difference (ASD) and the mean reciprocal ranks (MRR) for masculine and feminine words. If there is a large gap between the performances on test cases 
%A large gap of the results by the two versions indicates strong bias in the bilingual word embeddings.
%We test around 50 analogy pairs and collect the ranking difference between two forms as well as the similarity scores.  %For example, for ``university:professor = universidad:?'', we find that the rank of masculine form ``profesor'' is 1 with a similarity score of 0.80 while the rank of feminine form ``profesora'' is 5 with a similarity score of 0.66. So the similarity difference for  ``professor'' in Spanish is 0.14 and ranking difference is 4.

%\paragraph{Sentence Retrieval--Biased}
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/ES_EN_correlation.pdf}
	\vspace{-1em}
	\centering
	\caption{(M)WEAT scores for occupations in English and Spanish. For both axes, the smaller the number, the occupation is more leaning towards to female.}~\label{fig:ES_EN_corr}
	%\label{fig:boat1}
	\vspace{-2em}
\end{figure}

%\subsubsection{Utility Tests}
%\paragraph{Sentence Translation Retrieval}
%Following the evaluation of MUSE~\citet{conneau2017word}, we consider bag-of-words aggregation methods to perform sentence retrieval on the Europarl corpus. We consider 2k source sentence queries and 200k target sentences for each language pair and report the precision@k for k = 1, 5, 10. Each sentence is represented by the idf-weighted average of word embeddings.
\paragraph{Results}

Table~\ref{tab:bilingual_results} shows the results.  Results on word translation shows that the mitigation approaches do not harm the utility of bilingual word embedding and words in different languages still align well. 
From the results of word pair translation, the original bilingual embedding exhibits strong bias and the gap between two genders are around 0.49 in MRR in both ES-EN and FR-EN bilingual embeddings and the average cosine similarity difference is larger than 0.1. 
Hybrid\_Ori results in smallest difference for cosine similarity and MRR gap between two gender forms. However, the discrepancy between two forms is not completely removed.



To visualize the effect of bias mitigation, we project the bias-reduced embeddings of occupation words on the semantic gender direction as shown in Figure \ref{fig:viz_bilingual_before}.  Figure~\ref{fig:viz_bilingual_after} shows that after debiasing using Hybrid\_Ori, the two gender forms of occupation words are more symmteric with respect to the corresponding English embedding. 

%\kw{This should be a new subsection}
\subsection{Bias Correlation between Languages}
Finally, we compute the WEAT/MWEAT scores\footnote{We use WEAT score for English and MWEAT for Spanish. To show the direction of bias, we 
take out the outer absolute function in Eq. \eqref{eq:mweat}.} for each occupation and show the commonality and difference of gender bias between English and Spanish embedding. Results in Figure~\ref{fig:ES_EN_corr} shows that 
%For each occupation, we calculate the WEAT scorefor English Embedding and MWEAT score for Spainish and French
%if it is from English and calculate the MWEAT score if it is from a gendered languages. Note that we remove the final absolute value from the quantification of $b_w$ since we want to show the inclination of the occupations. We collect the scores for all the occupations and compute the Spearman's correlation and p-value between Spanish and English. 
%\paragraph{Results}
%\kw{If we have space, probably it's better to show all pair of three languages. Do we have some numbers (e.g., labor statistics) that we can coorelated this with ground truth? } 
%The results for bias correlation between languages are shown in Figure~\ref{fig:ES_EN_corr}, which presents the (M)WEAT scores for occupations in Spanish and English with some annotated with the English translation. The spearman correlation is 0.45 with a p-value of 0.0004, indicating the significance of the correlation. Specifically, we find that some 
occupations (``nurse'' and ``mathematician'') lean towards the same gender in both languages. However, some occupations (e.g., ``chef'') lean to different genders in different languages. In general, there is a strong correlation between gender bias in English and Spanish embedding (Spearman correlation=0.45 with p-value=0.0004). 

%, they are closer to male in English while closer to female in Spanish. This may be due to that in gendered languages, the female forms of the occupations associate with female concepts more than the male forms as shown in Section~\ref{analysis}, thus resulting in a negative MWEAT score which means inclination to the female side.

%\subsection{Results} \label{results}

%\kw{present Table 1 first and then show Figure.} 


% We test ``Mitigating-First'' and ``Shifting'' approaches introduced before. We also test the combination of the above two approaches, i.e., we first mitigate English, align English and Spanish, and shift words along \seg~direction as a post-processing step. We consider both zero and mitigated English words the neutral \emph{anchor} position. 

% From Table~\ref{tab:mono_results}, we can see that mitigating before alignment (De-Align) can significantly shorten the gap between two gender forms for the cross-lingual analogy task, while shifting along the semantic gender direction (Shift) is better at reducing the discrepancy in the WEAT association for two gender forms. 
% This is probably because that aligning Spanish words with the mitigated English words will make the two gender forms have similar distances to the corresponding English word. While shifting after alignment forces the embeddings of the two gender forms associate with each gender concepts more equally. 
% Overall the results suggest that a combination of the two approaches can benefit from both and (De-Shift (Ori)) can effectively mitigate the gender bias in ES or bilingual word embeddings according to the two tasks we consider.



==> EMNLP2019-Bias in Bilingual word embeddings/sections/intro.tex <==
Word embeddings are widely used in modern natural language processing tools. By virtue of their being trained on large, human-written corpora, recent studies have shown that word embeddings, in addition to capturing
a word's semantics, also encode gender bias in society~\cite{kaiwei,caliskan2017semantics}. As a result of this bias, the embeddings may cause undesired consequences in the resulting models~\cite{ZWYOC18, font2019equalizing}. Therefore, extensive effort has been put toward analyzing and mitigating gender bias in word embeddings \cite{kaiwei,zhao2018learning,dev2019attenuating,ethayarajh2019understanding}.
% Word embeddings are widely used in various NLP applications such as sentiment analysis, question answering, and coreference resolution. Despite the great success they bring to those applications, there are underlying stereotypes in those embeddings. People have analyzed bias in embeddings and proposed different methods to mitigate the bias~\cite{kaiwei,caliskan2017semantics}. However, they all focus on word embeddings in English (EN), where there is no grammatical gender~\cite{curzan2003gender}, i.e. most words do not have masculine or feminine forms~\cite{craig1986noun}.

Existing studies on gender bias almost exclusively focus on English (EN) word embeddings.
Unfortunately, the techniques used to mitigate bias in English word embeddings cannot be directly applied to languages with
%focuses on gender bias in English (EN) word embeddings. However, these methods for measuring and mitigating bias in English are not able to address gender bias in languages that contain
grammatical gender\footnote{Grammatical gender is a complicated linguistic phenomenon; many languages contain more than two gender classes. In this paper, we focus on languages with masculine and feminine classes. For gender in semantics, we follow the literature and address only binary gender.}, where all nouns are assigned a gender class and the corresponding dependent articles, adjectives, and verbs must agree in gender with the noun (e.g. in Spanish: \textit{la buena enfermera} the good female nurse, \textit{el buen enfermero} the good male nurse)~\cite{corbett1991gender,corbett2006agreement}.
%(e.g. in Spanish: el ni\~{n}o peque\~{n}o \textit{the small boy}, la ni\~{n}a peque\~{n}a \textit{the small girl})~\cite{corbett1991gender,corbett2006agreement}. 
%Languages with grammatical gender encode the masculine-feminine distinction as a grammatical feature. Personal nouns typically express a grammatical gender that aligns with the (perceived) sex of the referent, and dependent articles and adjectives must agree in gender with the noun (e.g. Spanish: el ni\ño peque˜no the small boy, la ni˜na peque˜na the small girl). Grammatical gender is marked on common nouns as well, extending the masculine-feminine distinction to inanimate referents without any apparent semantic basis for category membership.
%For example, the Spanish (ES) translations of ``lawyer'' can be ``abogado''(masculine) or ``abogada''(feminine), depending on the gender of the person described. 
This is because most existing approaches define bias in word embeddings based on the projection of a word on a gender direction (e.g. ``nurse'' in English is biased because its projection on the gender direction inclines towards  female). When the grammatical gender exists, such bias definition is problematic as masculine and feminine words naturally carry gender information. For example, ``enfermero'' (male nurse) and ``enfermera'' (female nurse) lean toward male and female, respectively. This is due to morphological agreement and should not be considered as a stereotype. 
%Moreover, for animate nouns like occupations, morphological agreement of gender for other parts in the sentences causes the embeddings of different gender forms of the same word inherently different, since word embeddings learn the representation of a word by the company it keeps~\cite{mikolov2013efficient}. \kw{Do we need this sentence? It seems to me redundant and convey the same idea as the previous sentence.}%This makes the gender information in Spanish more complicated than in English and it is much difficult for us to detect the bias in such languages.
%However, some languages like Spanish (ES) constitute grammatical gender\footnote{\url{https://en.wikipedia.org/wiki/Grammatical_gender}}. For example, the Spanish translations of ``lawyer'' can be ``abogado''(masculine) or ``abogada''(feminine), depending on the gender of the person described. But existing approaches for mitigating English word embeddings are not able to address gender bias in languages that contain grammatical gender. This is due to that most existing methods define bias based on the projection of the word on one gender direction (e.g. ``nurse'' is biased because its projection inclines towards the female side) and mitigate it by zeroing the gender projection of each word. When grammatical gender exists, the projection cannot be directly used to define bias since grammatical gender may cause the inclination, and this should not be considered as a stereotype.

% In this work, we analyze gender bias in languages where grammatical gender can be found and we focus on Spanish (ES).  For example, in ES, the reference for ``doctor''  can be ``doctor''(masculine) or ``doctora''(feminine) depending on the gender of the person described. The encoding of masculine-feminine distinction in grammar makes them different from EN and we need to propose different ways to measure and mitigate gender bias in these languages.

However, gender bias in the embeddings of languages with grammatical gender indeed exists. For example, when we align Spanish (ES) embeddings to English embeddings, the word ``abogado'' (male lawyer)  is closer to ``lawyer'' than ``abogada'' (female lawyer).
%a cross-lingual analogy test based on English-Spanish bilingual word embeddings obtained from aligning English and Spanish embeddings~\cite{conneau2017word}. 
%The failure to adapt to languages with grammatical gender of previous analysis also hinders gender bias analysis for their corresponding bilingual word embeddings. Cross-lingual analogy tests show that gender bias indeed exists in Spanish word embeddings and Engliash-Spanish bilingual word embeddings.
%However, we find that gender bias indeed exists in Spanish word embeddings and Engliash-Spanish bilingual word embeddings based on cross-lingual analogy tests.
%For example, the answer to the cross-lingual analogy: \emph{``law is to lawyer as ley (law) is to \underline{?}''} is ``abogado'' (male lawyer) with rank 1 and cosine similarity of 0.58 and ``abogada'' (female lawyer) with rank of 21 and similarity of 0.44. Note that we use the mitigated version of the English embedding from~\citet{kaiwei} to minimize the effect of gender bias from English embeddings. \kw{In the intro, we don't have to give details. Could we simplify this and say that when we aligned a debiased English embedding with a Spanish embedding, the word lawyer (English) is more closer to abogado than abgada?}
This observation implies a discrepancy in semantics between the masculine and feminine forms of the same occupation in Spanish word embeddings. A similar observation is also found in other languages, such as French (FR). 
%Such discrepancy will likely make downstream applications like machine translation that uses these embeddings produce biased results~\cite{font2019equalizing}. 

%Gender bias also exists in bilingual word embeddings for English and a language with grammatical gender as shown in~\ref{fig:viz_bilingual}. When projecting

In this paper, we refer languages that have gender distinctions for all nouns (e.g., Spanish and German) as \emph{gendered languages} and others that do not mark grammatical gender as \emph{languages without grammatical gender} (e.g., English). 
%\kw{Ryan, do you have a suggestion  for a better name?}
%we refer to languages with grammatical gender as \emph{gendered languages} and languages that does not mark grammatical gender as \emph{genderless languages}. 
We use Spanish and French as running examples and propose quantitative methods for evaluating bias in word embeddings of gendered languages and bilingual word embeddings that align a gendered language with English. 
%\footnote{Although English has distinct male and female pronouns, it has no distinction of grammatical gender for most nouns. \url{https://en.wikipedia.org/wiki/Genderless_language}}. 
We first define gender bias in the word embeddings of gendered languages by constructing two gender directions: the semantic gender direction and the grammatical gender direction. We then analyze gender bias in bilingual embeddings using a similar approach.
%After projecting occupation words with two gender forms on these directions, we find that masculine and feminine forms are mostly in a symmetric position on the grammatical gender direction but are asymmetric on the semantic gender direction, which shows the bias.

%To enable such analogy, we use pre-trained bilingual word embeddings for EN and ES from MUSE~\cite{conneau2017word} that aligns fasttext~\cite{fasttext} embeddings in a single vector space.

%We project occupation words with two gender forms and other nouns with one gender form on the two directions and find that masculine and feminine forms are mostly in a symmetric position on the grammatical gender direction but are asymmetric on the semantic gender direction. We also find some interesting case like the word ``perfume'', which is grammatically masculine but leaning towards female on the semantic gender direction.

To mitigate gender bias in these embeddings, we propose two approaches. One is shifting words along the semantic gender direction with respect to an anchor point and the other is mitigating English first and then aligning the embedding spaces. Results show that a hybrid of these two approaches effectively mitigate bias in Spanish and French word embeddings as well as ES-EN, FR-EN bilingual word embeddings. We also show through word similarity and word translation experiments that the utility of the original monolingual and bilingual word embeddings is preserved.

Our contributions are summarized in the following. (1) We show that word embeddings of gendered languages such as Spanish and French contain gender bias and bilingual word embeddings aligning these languages to English also inherit the bias. (2) Based on the observation, we propose new definitions of gender bias by constructing two gender directions. (3) We propose methods to reduce gender bias for both monolingual and bilingual embeddings and show that they effectively mitigate bias while preserving the original utility of embeddings. Source code and data are available at  \url{https://github.com/shaoxia57/Bias_in_Gendered_Languages}.%\jy{It seems 1,2 both talks about we find "gender bias" in ES,  do you talk about the new definition of gender directions? For 3, shouldn't the ``metric to evaluate the bias'' come  before your ``mitigate'' method? }
%To reduce the gap in the semantic gender information carried by the two gender forms, we compute offsets for each pair of words to shift them along the semantic gender direction. Furthermore, we explore mitigation methods by first debiasing monolingual word embeddings and then align them together in a common space. 


==> EMNLP2019-Bias in Bilingual word embeddings/sections/mitigation.tex <==

%We propose several simple yet effective methods for mitigating bias in gendered languages and bilingual word embeddings. 
In the following, we first describe the optimization objectives for mitigating gender bias. Then, we present mitigation methods under two settings: (1) \emph{monolingual setting}, where we only have access to word embeddings of the gendered language, and (2) \emph{bilingual setting}, where the embeddings of a language without grammatical gender (e.g. English) aligned in the same space are also provided.
%We design our methods for both the monolingual setting and the bilingual setting \jy{ duplicating the previous sentence?}. 
Specifically, for the bilingual setting, we can use English word vectors to facilitate the bias mitigation.
%\kw{When you say bilingual setting, do you thinking of using a language without grammar gender to facilitate the bias mitigation for a gendered langauge? If so, you want to make this clear. Otherwise, the Hybrid doesn't make sense as these are two different settings. }
\subsection{Mitigation Objectives}
%For nouns that only have one gender form, we follow the approach in \citet{kaiwei} and minimize the component of the word on the semantic gender direction. In particular, we project out the semantic gender component from inanimate nouns, as they should not carry semantic gender.
%components. %\jy{we  have 2 directions, so here should be semantic?}. 
%One important difference from the prior approach is that we use the semantic gender direction which is orthogonal to the grammatical gender to remove the effect of grammatical gender when quantifying bias. 
%We define the mitigation objective for inanimate nouns as:
For inanimate nouns, we project out their semantic gender component as they should not carry semantic gender. Equivalently, we minimize the inner product 

\begin{equation}
\label{eq:inanimate}
\left \langle \vec{w},\vec{d_s}  \right \rangle
\end{equation} between the inanimate word vector $\vec{w}$ and the semantic gender direction $\vec{d_s}$.
%\begin{equation*}
%\end{equation*}
%where $\vec{w}$ is embedding for the target word.
%\jy{Do you want to add description about the operation $\left \langle \vec{x},\vec{y}  \right \rangle$?}

For nouns with both gender forms, we aim at removing the gender inequality on the semantic gender direction as shown in Figure~\ref{fig:viz_2directions} and Figure~\ref{fig:viz_bilingual_before}. Specifically, we minimize the difference between the distance of feminine form of the word $\vec{w_f}$ and the masculine form of the word $\vec{w_m}$ to an anchor point (e.g., the origin point) on the semantic gender direciton $d_s$:
%most of which are used to describe people, we propose a new objective to mitigate the gender bias. 
%\kw{Give an example here. Also, how this definition is related to M-WEAT? We should also mention M-WEAT here, as it is also a metric to quantify the bias. Btw, the role of the anchor point is unclear here. }
%As shown in Figure~\ref{fig:viz_2directions} and Figure~\ref{fig:viz_bilingual_before}, the most severe discrepancy lies in the asymmetry on the semantic gender direction, i.e., most occupations in female form are farther away from the neutral position compared to those in male form. Thus we define the objective to computationally quantify this asymmetry. Furthermore, we define an anchor point that represents the gender-neutral position on the gender directions and a simple choice could be the origin point on the axis defined by the semantic gender direction. Let $\vec{w_f}$ be the word in feminine form, $\vec{w_m}$ be the word in masculine form, and $\vec{w_a}$ be the anchor point. We define the mitigation objective as:
\begin{equation}
\label{eq:objmf}
     \left | \left | \left \langle \vec{w}_m,\vec{d}_s  \right \rangle \!-\! \left \langle \vec{w}_a,\vec{d}_s  \right \rangle \right | \!-\!  \left | \left \langle \vec{w}_f,\vec{d}_s  \right \rangle \!-\! \left \langle \vec{w}_a,\vec{d}_s  \right \rangle \right | \right |.
\end{equation}
Note that for most cases, $\vec{w_m}$ and $\vec{w_f}$ lie on the opposite sides of the anchor point on the semantic gender axis. Therefore, we can simplify Eq. \eqref{eq:objmf} as
\begin{equation}
\label{eq:biasobj}
     \left | \left \langle \vec{w}_m,\vec{d}_s  \right \rangle + \left \langle \vec{w}_f,\vec{d}_s  \right \rangle - 2 \left \langle \vec{w}_a,\vec{d}_s  \right \rangle \right |.
\end{equation}

%$\left \langle \vec{w_m},\vec{d_s}  \right \rangle$ and $\left \langle \vec{w_f},\vec{d_s}  \right \rangle$ have opposite signs, meaning that the two forms lie on the opposite sides of the semantic gender axis.
%\jy{Maybe one sentence here to make it easier for the readers, saying the $\left \langle \vec{w_m},\vec{d_s}  \right \rangle$ and $\left \langle \vec{w_f},\vec{d_s}  \right \rangle$ have different +/- signs? }

Intuitively, this measures how much we need to move the word pair on the semantic gender direction so that they are symmetric with respect to the anchor point. If the anchor point is the origin point (i.e. $\left \langle \vec{w}_a,\vec{d}_s  \right \rangle=0$),  this objective is the absolute value of the sum of two projections.
%\kh{If you plan to use term "monolingual setting" and "bilingual setting", you can define them in sec 3. Then the paper will be more organized and the reader can have a mapping between sections.}
\subsection{Monolingual Setting}
\paragraph{Shifting Along Semantic Gender Direction (Shift)}
We mitigate bias by minimizing Eq. \eqref{eq:biasobj} and Eq. \eqref{eq:inanimate} in a post-processing manner. 
Effectively, for inanimate nouns, we remove the semantic gender component from the embeddings. For nouns with two gender forms (e.g., occupations),  
%by a post-processing step. Generally, we want the objectives to be zero. For inanimate nouns, we follow the previous work by~\citet{kaiwei} and mitigate by removing the semantic gender component from the embeddings. For animate nouns that have two gender forms like occupation terms, %instead of zeroing the projection of gender-neutral words on the gender direction, we want them to be symmetric on the semantic gender direction with respect to a neutral point.
we shift the two forms along the semantic gender direction so that they have the same distance to the anchor point.
%but are on the opposite sides, which also effectively makes the objective for animate nouns zero.
For monolingual setting, we use the origin point on the gender direction as the anchor point and call the method Shift\_Ori.
%\kh{Do you mean $b_w$? If yes, you don't need to explain it so much. Instead, you can say previous work can let $b_w$ of gender-neutral inanimate nouns be zero. And then talk about how we let $b_w$ of two gender form nouns be zero.}
%We consider two types of anchor positions: the zero point of the gender axis and the projection of the mitigated English word using ``hard-debiasing'' approach in the bilingual word embeddings. 

Note that \citet{gonen2019lipstick} show that mitigating gender bias in word embeddings by moving on the gender direction is not sufficient and words with gender bias still tend to group together. Similairly, our approach might not entirely remove the gender bias. However, the approach in \citet{gonen2019lipstick} to test the remainder bias cannot be applied directly for gendered languages, because grouping of the embeddings of masculine and feminine words does not always indicate bias due to grammatical gender .
%argue that for languages with grammatical gender, and shifting words on the semantic gender direction is able to mitigate gender bias using our proposed metrics shown in Section~\ref{results}. \kw{I'm not sure if I understand the argument. I think we have to say that  ...  }

\subsection{Bilingual Setting}
\paragraph{Mitigating Before Alignment (De-Align)}
As gender bias can be observed when aligning gendered languages with language without grammatical gender, we consider using English to facilitate mitigating bias. Specifically, we first apply the ``hard-debasing'' approach~\citet{kaiwei} to English embedding and then align gendered language with the bias-reduced English. Because most words with both gender forms align to the same word in English (e.g., ``enfermero'' and ``enfermera'' in Spanish both align to ``nurse'' in English), the alignment places the two gender forms of the words in a more symmetric positions in the vector space after the alignment. 
%Although mitigation methods for word embeddings of gendered languages are underexplored, many approaches have been proposed for English and they could be helpful for mitigating gender bias in the bilingual embedding setting. We mitigate bias in bilingual word embeddings that align English with a gendered language by first mitigating the English word embedding following the ``hard-debiasing'' approach from~\citet{kaiwei} and then aligning the two languages in a single vector space. The intuition of mitigating gender bias in English before alignment is that it could potentially align the Spanish words with the less biased English embeddings and thus make the two gender forms of the Spanish terms in more symmetric positions in the vector space.% After alignment, we can treat Spanish words in bilingual word embeddings as our mitigated Spanish word embeddings.
%The first method mitigates gender bias as a post-processing step. We also consider debiasing EN embedding before aligning them with ES embeddings. 
\paragraph{Shifting Along Semantic Gender Direction (Shift)}
We consider using English words as anchor positions when mitigating bias using Eq \eqref{eq:biasobj}. We call this approach Shift\_EN. For example, when applying Eq. \eqref{eq:biasobj} to re-position ``enfermero'' and ``enfermera'' in Spanish we take English word ``nurse'' aligned in the same space as the anchor position. 

%This approach is the same as our proposed method for the monolingual setting, except that we can also treat the bias-mitigated English word embeddings as the anchor position (Shift\_EN) because we have the English word embeddings aligned in the same space.
%kw{I don't understand the difference between Shift and Hybrid\_EN}
\paragraph{Hybrid Method (Hybrid)}
We also consider a hybrid method that integrates the aforementioned two approaches.
%above for the bilingual setting because we find that the two mitigation methods are applied to the bilingual embeddings at different times, i.e. before and after alignment. 
In particular, we first mitigate English embeddings, align English embeddings with the embeddings of gendered languages, and then shift words in languages with grammatical gender along the semantic gender direction. 
We consider two variants based on how the anchor positions are chosen: (1) Hybrid\_Ori uses the origin point as the anchor position; and (2) Hybrid\_EN uses the corresponding bias-reduced English word as an anchor position when shifting a pair of words with different gender forms. 

%with two choices of anchor positions: origin point (Hybrid\_Ori) and mitigated English words (Hybrid\_EN).

%\kh{Why we don't try Shifting with Origin as Anchor?}

%\paragraph{Combination of Mitigation Before and After Alignment}
%he two methods proposed above are designed for separate stages: before and after alignment, so we can combine them together and hope that they can complement each other to better mitigate bias.

==> EMNLP2019-Bias in Bilingual word embeddings/sections/mono_table.tex <==
\begin{table*}[ht]
\centering
%\small
\begin{tabularx}{\linewidth}{c|c||c||c|c|c|c|c}
Lang. & Metric         & Original       & Shift\_Ori    & Shift\_EN     & De-Align & Hybrid\_Ori    & Hybrid\_EN \\ \hline
%ES--WEAT--Male      & 0.052          & 0.086          & \textbf{0.083} & 0.052    & 0.086          & 0.063      \\
%ES--WEAT--Female    & 0.115          & 0.081          & \textbf{0.084} & 0.115    & 0.081          & 0.103      \\
ES & MWEAT--Diff      & 3.6918          & 0.3090          & 0.3324 & 3.5748    & \textbf{0.3090}          & 2.2494      \\ 
ES & MWEAT--p-value    & 0.0000          & 0.1130          & 0.0010  & 0.0010   & \textbf{0.7330}          & 0.0020     \\ \hline
%FR--WEAT--Male      & 0.055          & \textbf{0.122} & 0.105          & 0.055    & \textbf{0.122} & 0.085      \\
%FR--WEAT--Female    & 0.185          & \textbf{0.118} & 0.135          & 0.185    & \textbf{0.118} & 0.155      \\
FR & MWEAT--Diff      & 2.3437          & 0.2446 & 0.3882          & 2.3436    & \textbf{0.2446} & 1.1758      \\ 
FR & MWEAT--p-value    & 0.0000          & 0.1470 & 0.0010          & 0.0020    & \textbf{0.5290} & 0.0910      \\ \hline
ES & Word Similarity & \textbf{0.7392} & 0.7363          & 0.7359         & \textbf{0.7392}    & 0.7358          & 0.7356      \\
FR & Word Similarity & \textbf{0.7294} & 0.7218          & 0.7218         & 0.7156    & 0.7218          & 0.7218     
\end{tabularx}
\caption{Analyses on Spanish and French monolingual embeddings before and after bias mitigation. Results show that the original Spanish and French embeddings exhibit strong bias and Hybrid\_Ori significantly reduces the bias in the embedding to to an insignificant level (p-value $>$ 0.05).}
%We find the original MWEAT p-value to be 0, which indicates gap in the two forms of gender. Hybrid method with origin as anchor can largely decrease the MWEAT difference and increase the p-value to much higher than the statistical significance threshold (0.05). We also report results from word similarity tests that show that our methods preserve the quality.}%
\label{tab:mono_results}
\end{table*}


% \begin{table*}[ht]
% \begin{tabularx}{\linewidth}{c|c|c|c|c|c|c}
% \hline
%                          & Original & \begin{tabular}[c]{@{}c@{}}Shift (Ori) \end{tabular} & \begin{tabular}[c]{@{}c@{}}Shift (EN) \end{tabular} & \begin{tabular}[c]{@{}c@{}}De-Align \end{tabular} & \begin{tabular}[c]{@{}c@{}}De-Shift (Ori) \end{tabular} & \begin{tabular}[c]{@{}c@{}}De-Shift (EN)\end{tabular} \\ \hline
% CLAT--ASD      & 0.1244  & 0.1024                                                                 & 0.0978                                                                      & 0.0735                                                              & 0.0642                                                                                 & \textbf{0.0586}                                                                    \\ \hline
% CLAT--ARD      & 17.8413 & 15.3968                                                                & 14.8413                                                                     & 1.6984                                                               & \textbf{1.6191}                                                                        & \textbf{1.6191}                                                                    \\ \hline
% WEAT--Male   & 0.4633  & 0.9245                                                                 & \textbf{0.9010}                                                             & 0.4633                                                               & 0.9254                                                                                 & 0.5699                                                                             \\ \hline
% WEAT--Female & 1.3339 & 0.87272                                                               & \textbf{0.8962}                                                            & 1.3339                                                              & 0.8718                                                                                & 1.2273                                                                            \\ \hline
% \end{tabularx}
% \caption{Results for different bias mitigation methods on two types of evaluation metrics. ``CLAT'' stands for cross-lingual analogy task, ``ASD'' is the average similarity difference for masculine and feminine words, ``ARD'' is the average ranking difference, ``WEAT--Male'' is the association of male occupation words with male-definition terms subtracting that with female-definition, similarly for ``WEAT--Female'', ``Shift (Ori)'' is the debiasing method of shifting along the semantic gender direction with the zero point as anchors, similarly for ``Shift (EN)'', which treats the debiased EN counterparts as anchors, ``De-Align'' is first debias EN and then align, and ``De-Shift (Ori)'' is the method combining first debiasing then align and shifting along semantic direction with the origin as anchor as post-processing.}%
% \label{tab:results}
% \end{table*}

==> EMNLP2019-Bias in Bilingual word embeddings/sections/related_work.tex <==
Previous work has proposed to quantify bias in English Embedding
definitions for gender bias in English word embeddings. 
%\citet{kaiwei} define  a gender direction using the difference between male- and female-definition word embeddings and show that occupational words have different distances to ``male'' or ``female'' on this direction. This is appropriate for English as it does not distinguish between the masculine and feminine forms for most nouns but not applicable for gendered languages as mentioned earlier. %However, in languages with grammatical gender, all nouns are assigned with a grammatical gender, and the gender information in such words does not necessarily indicate that the words are semantically towards one gender.
%including those inanimate objects such as ``table'' and ``apple''. 
%\kh{It seems that the reason is not straightforward for me. Previous work uses occupational words to show the bias. So maybe using some occupational words as examples rather than table and apple is better?}
Besides the aforementioned studies~\cite{kaiwei,caliskan2017semantics} in quantifying bias in English embedding,
\citet{katherine2017grammatical} examine grammatical gender bias in word embeddings of gendered languages by computing the WEAT association score~\cite{caliskan2017semantics} between gendered object nouns (e.g. moon-sun) and gender-definition words.
They propose to mitigate bias by applying lemmatization to remove gender information from the training corpus.
However, their focus is different from us as our approaches aim at keeping the grammatical gender information and only removing the bias in semantic genders. 
%However, we argue that the association between gendered object nouns with gender attributes should not be considered as stereotypical bias since the association could be caused by the morphological agreement instead of stereotypes. Mitigation by completely removing gender information is also implausible as too much information will be lost by lemmatization.
A few recent studies focus on measuring and reducing gender bias in contextualized word embeddings~\cite{ZWYCOC19,may2019measuring,basta2019evaluating}. 
However, they only focus on English embeddings in which the gender is mostly only expressed by pronouns~\cite{stahlberg2007representation}.
An interesting future direction is to extend their analyses to language with grammatical gender. 

Regarding bias mitigation appraoches, \citet{zhao2018learning} mitigate bias by saving one dimension of the word vector for gender.~\citet{bordia2019identifying} propose a regularization loss term for word-level language models.~\citet{zhang2018mitigating} use an adversarial network to mitigate bias in word embeddings. All these approaches consider only English embeddings. Moreover,~\citet{gonen2019lipstick} show that mitigation methods based on gender directions are not sufficient, since the embeddings of socially-biased words still cluster together.

%\jy{Changed the order in this section to: 1 talk about measuring bias in worde embeddings; 2 mitigate such bias ; 3 other applications. I haven't checked the other papers, but for \citet{zhao2018learning}, it can add another dimension to preserve the grammatical gender. So in the last sentence, you may want to make sure about `` they cannot be applied to languages with grammatical gender''}

%Bias outside word embeddings
Bias in word embedding may affect the downstream applications~\cite{ZWYOC18,rudinger2018gender,font2019equalizing}.
%\jy{This sentcence doesn't align with the contextualized word embeddings. maybe we can move to this part?}
Besides the gender bias in word embeddings, implicit stereotypes have been shown in other real world applications, such as online reviews~\cite{wallace2016jerk}, advertisement~\cite{sweeney2013discrimination} and web search~\cite{kay2015unequal}. 
%Dataset bias~\cite{jieyu,rudinger2017social} and word embedding bias~\cite{kaiwei,caliskan2017semantics} both contribute to this problem.
%while this work focuses on the later part, specifically for gendered languages.
